Enforcing Operational Properties including Blockfreeness for Deterministic Pushdown Automata

We present an algorithm which modifies a deterministic pushdown automaton (DPDA) such that (i) the marked language is preserved, (ii) lifelocks are removed, (iii) deadlocks are removed, (iv) all states and edges are accessible, and (v) operational blockfreeness is established (i.e., coaccessibility in the sense that every initial derivation can be continued to a marking configuration). This problem can be trivially solved for deterministic finite automata (DFA) but is not solvable for standard petri net classes. The algorithm is required for an operational extension of the supervisory control problem (SCP) to the situation where the specification in modeled by a DPDA.

==> figures/fig__example__NFA.tex <==
\begin{tikzpicture}[SFSautomatX,on grid,node distance=.85cm]
\node[initial text=,initial where=above,istate,inner sep=1pt,minimum size=0cm] (q0) at (0,0) {$q_0$};
\node[state,inner sep=1pt,minimum size=0cm] (q1) [right=of q0] {$q_1$};
\node[fstate,inner sep=1pt,minimum size=0cm] (q2) [left=of q0] {$q_2$};

\SFSAutomatEdge{q0}{a}{q1}{swap}{}
\SFSAutomatEdge{q0}{a}{q2}{}{}
\end{tikzpicture}

==> figures/fig__example__Parser0.tex <==
\centering%
\def\widthB{.65}%
\def\widthC{.25}%
\adjustbox{valign=t}{\begin{minipage}[t]{\widthB\linewidth}
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l@{\;\;\;\;}r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{8}{l}{\text{Reduce Rules}}\\
\midrule
% \RULESepCol{1\sconc3\sconc5}{\ENDOFOUTPUT}{1\sconc6}{\ENDOFOUTPUT} &
1\sconc3\sconc5&\ENDOFOUTPUT&1\sconc6&\ENDOFOUTPUT &
1\sconc2\sconc7&\ENDOFOUTPUT&1\sconc6&\ENDOFOUTPUT\\
2\sconc8\sconc10&\ENDOFOUTPUT&2\sconc7&\ENDOFOUTPUT &
2\sconc9\sconc12&\ENDOFOUTPUT&2\sconc8&\ENDOFOUTPUT\\
3\sconc4&\ENDOFOUTPUT&3\sconc5&\ENDOFOUTPUT &
3&\ENDOFOUTPUT&3\sconc4&\ENDOFOUTPUT\\
8\sconc4&\ENDOFOUTPUT&8\sconc10&\ENDOFOUTPUT &
8&\ENDOFOUTPUT&8\sconc4&\ENDOFOUTPUT\\
9\sconc13\sconc16&\ENDOFOUTPUT&9\sconc12&\ENDOFOUTPUT &
13\sconc17\sconc18&\ENDOFOUTPUT&13\sconc16&\ENDOFOUTPUT\\
17&\ENDOFOUTPUT&17\sconc18&\ENDOFOUTPUT &
9\sconc14\sconc19&d&9\sconc13&d\\
9\sconc15\sconc22&d&9\sconc13&d &
14\sconc26\sconc27&d&14\sconc19&d\\
% 14\sconc20\sconc21&d&14\sconc19&d\\
15\sconc23\sconc25&d&15\sconc22&d&
15\sconc24\sconc28&b&15\sconc23&b\\
% 20&d&20\sconc21&d &
23\sconc26\sconc27&d&23\sconc25&d\\
24\sconc29\sconc30&b&24\sconc28&b &
24\sconc15\sconc22&d&24\sconc29&d\\
24\sconc14\sconc19&d&24\sconc29&d &
26&d&26\sconc27&d\\
29\sconc31\sconc32&b&29\sconc30&b &
31&b&31\sconc32&b\\
\bottomrule
\end{array}$
\end{minipage}}%
\adjustbox{valign=t}{\begin{minipage}[t]{\widthC\linewidth}
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{3}{l}{\text{Shift Rules}}\\
\midrule
1&a&1\sconc2&\\
1&b&1\sconc3&\\
2&a&2\sconc9&\\
9&a&9\sconc15&\\
9&b&9\sconc14&\\
13&d&13\sconc17&\\
14&b&14\sconc26&\\
15&a&15\sconc24&\\
23&b&23\sconc26&\\
24&a&24\sconc15&\\
24&b&24\sconc14&\\
29&d&29\sconc31&\\
\bottomrule
\end{array}$
\end{minipage}}%


==> figures/fig__example__Parser1.tex <==
\centering%
\def\widthB{.65}%
\def\widthC{.25}%
\adjustbox{valign=t}{\begin{minipage}[t]{\widthB\linewidth}
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l@{\;\;\;\;}r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{8}{l}{\text{Reduce Rules}}\\
\midrule
% \RULESepCol{1\sconc3\sconc5}{\$}{1\sconc6}{\$} &
9\sconc14\sconc19&d&9\sconc13&d &
24\sconc14\sconc19&d&24\sconc29&d \\
9\sconc15\sconc22&d&9\sconc13&d &
24\sconc15\sconc22&d&24\sconc29&d \\
15\sconc23\sconc25&d&15\sconc22&d &
26&d&26\sconc27&d \\
14\sconc26\sconc27&d&14\sconc19&d &
23\sconc26\sconc27&d&23\sconc25&d \\
15\sconc24\sconc28&b&15\sconc23&b &
24\sconc29\sconc30&b&24\sconc28&b \\
31&b&31\sconc32&b &
29\sconc31\sconc32&b&29\sconc30&b \\
\bottomrule
\end{array}$
\end{minipage}}%
\adjustbox{valign=t}{\begin{minipage}[t]{\widthC\linewidth}
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{3}{l}{\text{Shift Rules}}\\
\midrule
1&a&1\sconc2&\\
1&b&1\sconc3&\\
2&a&2\sconc9&\\
9&a&9\sconc15&\\
9&b&9\sconc14&\\
13&d&13\sconc17&\\
14&b&14\sconc26&\\
15&a&15\sconc24&\\
23&b&23\sconc26&\\
24&a&24\sconc15&\\
24&b&24\sconc14&\\
29&d&29\sconc31&\\
\bottomrule
\end{array}$
\end{minipage}}%


==> figures/fig__example__Parser2.tex <==
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l@{\;\;\;\;}r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{8}{l}{\text{Reduce Rules}}\\
\midrule
% \RULESepCol{1\sconc3\sconc5}{\$}{1\sconc6}{\$} &
9\sconc14\sconc(19,\EMPTYSTRING)&d&9\sconc(13,d)&\EMPTYSTRING&
9\sconc14\sconc(19,d)&\EMPTYSTRING&9\sconc(13,d)&\EMPTYSTRING\\
24\sconc14\sconc(19,\EMPTYSTRING)&d&24\sconc(29,d)&\EMPTYSTRING&
24\sconc14\sconc(19,d)&\EMPTYSTRING&24\sconc(29,d)&\EMPTYSTRING\\
9\sconc15\sconc(22,\EMPTYSTRING)&d&9\sconc(13,d)&\EMPTYSTRING&
9\sconc15\sconc(22,d)&\EMPTYSTRING&9\sconc(13,d)&\EMPTYSTRING\\
24\sconc15\sconc(22,\EMPTYSTRING)&d&24\sconc(29,d)&\EMPTYSTRING&
24\sconc15\sconc(22,d)&\EMPTYSTRING&24\sconc(29,d)&\EMPTYSTRING\\
15\sconc23\sconc(25,\EMPTYSTRING)&d&15\sconc(22,d)&\EMPTYSTRING&
15\sconc23\sconc(25,d)&\EMPTYSTRING&15\sconc(22,d)&\EMPTYSTRING\\
(26,\EMPTYSTRING)&d&26\sconc(27,d)&\EMPTYSTRING&
(26,d)&\EMPTYSTRING&26\sconc(27,d)&\EMPTYSTRING\\
14\sconc26\sconc(27,\EMPTYSTRING)&d&14\sconc(19,d)&\EMPTYSTRING&
14\sconc26\sconc(27,d)&\EMPTYSTRING&14\sconc(19,d)&\EMPTYSTRING\\
23\sconc26\sconc(27,\EMPTYSTRING)&d&23\sconc(25,d)&\EMPTYSTRING&
23\sconc26\sconc(27,d)&\EMPTYSTRING&23\sconc(25,d)&\EMPTYSTRING\\
15\sconc24\sconc(28,\EMPTYSTRING)&b&15\sconc(23,b)&\EMPTYSTRING&
15\sconc24\sconc(28,b)&\EMPTYSTRING&15\sconc(23,b)&\EMPTYSTRING\\
24\sconc29\sconc(30,\EMPTYSTRING)&b&24\sconc(28,b)&\EMPTYSTRING&
24\sconc29\sconc(30,b)&\EMPTYSTRING&24\sconc(28,b)&\EMPTYSTRING\\
(31,\EMPTYSTRING)&b&31\sconc(32,b)&\EMPTYSTRING&
(31,b)&\EMPTYSTRING&31\sconc(32,b)&\EMPTYSTRING\\
29\sconc31\sconc(32,\EMPTYSTRING)&b&29\sconc(30,b)&\EMPTYSTRING&
29\sconc31\sconc(32,b)&\EMPTYSTRING&29\sconc(30,b)&\EMPTYSTRING\\
\bottomrule
\end{array}$\\
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l@{\;\;\;\;}r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{3}{l}{\text{Shift Rules}}\\
\midrule
(1,\EMPTYSTRING)&a&1\sconc(2,\EMPTYSTRING)&\EMPTYSTRING&
(1,a)&\EMPTYSTRING&1\sconc(2,\EMPTYSTRING)&\EMPTYSTRING\\
(1,\EMPTYSTRING)&b&1\sconc(3,\EMPTYSTRING)&\EMPTYSTRING&
(1,b)&\EMPTYSTRING&1\sconc(3,\EMPTYSTRING)&\EMPTYSTRING\\
(2,\EMPTYSTRING)&a&2\sconc(9,\EMPTYSTRING)&\EMPTYSTRING&
(2,a)&\EMPTYSTRING&2\sconc(9,\EMPTYSTRING)&\EMPTYSTRING\\
(9,\EMPTYSTRING)&a&9\sconc(15,\EMPTYSTRING)&\EMPTYSTRING&
(9,a)&\EMPTYSTRING&9\sconc(15,\EMPTYSTRING)&\EMPTYSTRING\\
(9,\EMPTYSTRING)&b&9\sconc(14,\EMPTYSTRING)&\EMPTYSTRING&
(9,b)&\EMPTYSTRING&9\sconc(14,\EMPTYSTRING)&\EMPTYSTRING\\
(13,\EMPTYSTRING)&d&13\sconc(17,\EMPTYSTRING)&\EMPTYSTRING&
(13,d)&\EMPTYSTRING&13\sconc(17,\EMPTYSTRING)&\EMPTYSTRING\\
(14,\EMPTYSTRING)&b&14\sconc(26,\EMPTYSTRING)&\EMPTYSTRING&
(14,b)&\EMPTYSTRING&14\sconc(26,\EMPTYSTRING)&\EMPTYSTRING\\
(15,\EMPTYSTRING)&a&15\sconc(24,\EMPTYSTRING)&\EMPTYSTRING&
(15,a)&\EMPTYSTRING&15\sconc(24,\EMPTYSTRING)&\EMPTYSTRING\\
(23,\EMPTYSTRING)&b&23\sconc(26,\EMPTYSTRING)&\EMPTYSTRING&
(23,b)&\EMPTYSTRING&23\sconc(26,\EMPTYSTRING)&\EMPTYSTRING\\
(24,\EMPTYSTRING)&a&24\sconc(15,\EMPTYSTRING)&\EMPTYSTRING&
(24,a)&\EMPTYSTRING&24\sconc(15,\EMPTYSTRING)&\EMPTYSTRING\\
(24,\EMPTYSTRING)&b&24\sconc(14,\EMPTYSTRING)&\EMPTYSTRING&
(24,b)&\EMPTYSTRING&24\sconc(14,\EMPTYSTRING)&\EMPTYSTRING\\
(29,\EMPTYSTRING)&d&29\sconc(31,\EMPTYSTRING)&\EMPTYSTRING&
(29,d)&\EMPTYSTRING&29\sconc(31,\EMPTYSTRING)&\EMPTYSTRING\\
\bottomrule
\end{array}$
% \end{minipage}}%


==> figures/fig__example__derivation_SDPDA_LR1G.tex <==
$\begin{array}{ll|ll}
\toprule
\multicolumn{2}{l}{\;\;\SDPDA~\STEP{2}}&\multicolumn{2}{l}{\;\;\LR~\STEP{4}}\\
\midrule
  &(\STATEELEM_0,\EMPTYSTRING,\Box)&
  &L_{\STATEELEM_0,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_0',a,\Box)&  
\DERIVE{\STEP{4}}&
  a\sconc L_{\STATEELEM_0',\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_0,a,\bullet\Box)&
\DERIVE{\STEP{4}}&
  a\sconc L_{\STATEELEM_0,\bullet,\STATEELEM_1}\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_0'',aa,\bullet\Box)&
\DERIVE{\STEP{4}}&
  aa\sconc L_{\STATEELEM_0'',\bullet,\STATEELEM_1}\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_0,aa,\bullet\bullet\Box)&
\DERIVE{\STEP{4}}&
  aa\sconc L_{\STATEELEM_0,\bullet,\STATEELEM_2}\sconc L_{\STATEELEM_2,\bullet,\STATEELEM_1}\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_1,aab,\bullet\bullet\Box)&
\DERIVE{\STEP{4}}&
  aab\sconc L_{\STATEELEM_1,\bullet,\STATEELEM_2}\sconc L_{\STATEELEM_2,\bullet,\STATEELEM_1}\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_1',aabb,\bullet\bullet\Box)&
\DERIVE{\STEP{4}}&
  aabb\sconc L_{\STATEELEM_1',\bullet,\STATEELEM_2}\sconc L_{\STATEELEM_2,\bullet,\STATEELEM_1}\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_2,aabb,\bullet\Box)&
\DERIVE{\STEP{4}}&
  aabb\sconc L_{\STATEELEM_2,\bullet,\STATEELEM_1}\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_2',aabbd,\bullet\Box)&
\DERIVE{\STEP{4}}&
  aabbd\sconc L_{\STATEELEM_2',\bullet,\STATEELEM_1}\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_1,aabbd,\Box)&
\DERIVE{\STEP{4}}&
  aabbd\sconc L_{\STATEELEM_1,\Box}\\
\DERIVE{\STEP{2}}&
  (\STATEELEM_3,aabbd,\bullet\Box)&
\DERIVE{\STEP{4}}&
  aabbd\sconc L_{\STATEELEM_3,\bullet}\\
  &&
\DERIVE{\STEP{4}}&
  aabbd\\
\bottomrule
\end{array}$

==> figures/fig__example__derivation_SDPDA_LRP.tex <==
$\begin{array}{ll|ll}
\toprule
\multicolumn{2}{l}{\;\;\SDPDA~M_2'}&\multicolumn{2}{l}{\;\;\text{Parser}~P_0}\\
\midrule
  &(q_0,\EMPTYSTRING,\Box)&
  &(1,\EMPTYSTRING,\EMPTYSTRING)\\
  
\DERIVE{M_2'}&
  (q_0',a,\Box)&  
\DERIVE{P_0}&
  (1\sconc2,a,\EMPTYSTRING)\\
  
\DERIVE{M_2'}&
  (q_0,a,\bullet\Box)&
  &\\
  
\DERIVE{M_2'}&
  (q_0'',aa,\bullet\Box)&
\DERIVE{P_0}&
  (1\sconc2\sconc9,aa,\EMPTYSTRING)\\
  
\DERIVE{M_2'}&
  (q_0,aa,\bullet\bullet\Box)&
  &\\
  
\DERIVE{M_2'}&
  (q_1,aab,\bullet\bullet\Box)&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc14,aab,\EMPTYSTRING)\\  
  
\DERIVE{M_2'}&
  (q_1',aabb,\bullet\bullet\Box)&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc14\sconc20,aabb,\EMPTYSTRING)\\  
  
\DERIVE{M_2'}&
  (q_2,aabb,\bullet\Box)&
  &\\

\DERIVE{M_2'}&
  (q_2',aabbd,\bullet\Box)&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc14\sconc20\sconc21,aabbd,d)\\
  
  &&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc14\sconc19,aabbd,d)\\
  
  &&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc13,aabbd,d)\\ 

  &&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc13\sconc17,aabbd,\EMPTYSTRING)\\ 
  
\DERIVE{M_2'}&
  (q_1,aabbd,\Box)&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc13\sconc17\sconc18,aabbd,\$)\\ 
  
\DERIVE{M_2'}&
  (q_3,aabbd,\bullet\Box)&
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc13\sconc16,aabbd,\$)\\ 
  
  &&  
\DERIVE{P_0}&
  (1\sconc2\sconc9\sconc12,aabbd,\$)\\

  &&  
\DERIVE{P_0}&
  (1\sconc2\sconc8,aabbd,\$)\\
  
  &&  
\DERIVE{P_0}&
  (1\sconc2\sconc8\sconc4,aabbd,\$)\\
  
  &&  
\DERIVE{P_0}&
  (1\sconc2\sconc8\sconc10,aabbd,\$)\\
  
  &&  
\DERIVE{P_0}&
  (1\sconc2\sconc7,aabbd,\$)\\
  
  &&  
\DERIVE{P_0}&
  (1\sconc6,aabbd,\$)\\
\bottomrule
\end{array}$


==> figures/fig__example__derivation_SDPDA_LRP_dollarFree.tex <==
$\begin{array}{ll|ll}
\toprule
\multicolumn{2}{l}{\;\;\SDPDA~M_2'}&\multicolumn{2}{l}{\;\;\text{Parser}~P_1}\\
\midrule
  &(q_0,\EMPTYSTRING,\Box)&
  &(1,\EMPTYSTRING,\EMPTYSTRING)\\
  
\DERIVE{M_2'}&
  (q_0',a,\Box)&  
\DERIVE{P_1}&
  (1\sconc2,a,\EMPTYSTRING)\\
  
\DERIVE{M_2'}&
  (q_0,a,\bullet\Box)&
  &\\
  
\DERIVE{M_2'}&
  (q_0'',aa,\bullet\Box)&
\DERIVE{P_1}&
  (1\sconc2\sconc9,aa,\EMPTYSTRING)\\
  
\DERIVE{M_2'}&
  (q_0,aa,\bullet\bullet\Box)&
  &\\
  
\DERIVE{M_2'}&
  (q_1,aab,\bullet\bullet\Box)&
\DERIVE{P_1}&
  (1\sconc2\sconc9\sconc14,aab,\EMPTYSTRING)\\  
  
\DERIVE{M_2'}&
  (q_1',aabb,\bullet\bullet\Box)&
\DERIVE{P_1}&
  (1\sconc2\sconc9\sconc14\sconc20,aabb,\EMPTYSTRING)\\  
  
\DERIVE{M_2'}&
  (q_2,aabb,\bullet\Box)&
  &\\

\DERIVE{M_2'}&
  (q_2',aabbd,\bullet\Box)&
\DERIVE{P_1}&
  (1\sconc2\sconc9\sconc14\sconc20\sconc21,aabbd,d)\\
  
\DERIVE{M_2'}&
  (q_1,aabbd,\Box)&
\DERIVE{P_1}&
  (1\sconc2\sconc9\sconc14\sconc19,aabbd,d)\\
  
\DERIVE{M_2'}&
  (q_3,aabbd,\bullet\Box)&
\DERIVE{P_1}&
  (1\sconc2\sconc9\sconc13,aabbd,d)\\ 

  &&
\DERIVE{P_1}&
  (1\sconc2\sconc9\sconc13\sconc17,aabbd,\EMPTYSTRING)\\ 
\bottomrule
\end{array}$


==> figures/fig__example__essentiallyEDPDA.tex <==
\centering%
\def\widthB{.45}%
\def\widthC{.45}%
\adjustbox{valign=t}{\begin{minipage}[t]{\widthB\linewidth}
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{3}{l}{\text{Reduce Rules}}\\
\midrule
(9)(14)(19,\EMPTYSTRING)&d&(9)(13,d)&\\
(9)(14)(19,d)&\EMPTYSTRING&(9)(13,d)&\\
(9)(15)(22,\EMPTYSTRING)&d&(9)(13,d)&\\
(9)(15)(22,d)&\EMPTYSTRING&(9)(13,d)&\\
(14)(20)(21,\EMPTYSTRING)&d&(14)(19,d)&\\
(14)(20)(21,d)&\EMPTYSTRING&(14)(19,d)&\\
(15)(23)(25,\EMPTYSTRING)&d&(15)(22,d)&\\
(15)(23)(25,d)&\EMPTYSTRING&(15)(22,d)&\\
(15)(24)(28,\EMPTYSTRING)&b&(15)(23,b)&\\
(15)(24)(28,b)&\EMPTYSTRING&(15)(23,b)&\\
(20,\EMPTYSTRING)&d&(20)(21,d)&\\
(20,d)&\EMPTYSTRING&(20)(21,d)&\\
(23)(26)(27,\EMPTYSTRING)&d&(23)(25,d)&\\
(23)(26)(27,d)&\EMPTYSTRING&(23)(25,d)&\\
(24)(29)(30,\EMPTYSTRING)&b&(24)(28,b)&\\
(24)(29)(30,b)&\EMPTYSTRING&(24)(28,b)&\\
(24)(15)(22,\EMPTYSTRING)&d&(24)(29,d)&\\
(24)(15)(22,d)&\EMPTYSTRING&(24)(29,d)&\\
(24)(14)(19,\EMPTYSTRING)&d&(24)(29,d)&\\
(24)(14)(19,d)&\EMPTYSTRING&(24)(29,d)&\\
(26,\EMPTYSTRING)&d&(26)(27,d)&\\
(26,d)&\EMPTYSTRING&(26)(27,d)&\\
(29)(31)(32,\EMPTYSTRING)&b&(29)(30,b)&\\
(29)(31)(32,b)&\EMPTYSTRING&(29)(30,b)&\\
(31,\EMPTYSTRING)&b&(31)(32,b)&\\
(31,b)&\EMPTYSTRING&(31)(32,b)&\\
\bottomrule
\end{array}$
\end{minipage}}%
\adjustbox{valign=t}{\begin{minipage}[t]{\widthC\linewidth}
$\begin{array}{r@{|}l@{\rightarrow}r@{|}l}
\toprule
\multicolumn{3}{l}{\text{Shift Rules}}\\
\midrule
(1,\EMPTYSTRING)&a&(1)(2,\EMPTYSTRING)&\\
(1,a)&\EMPTYSTRING&(1)(2,\EMPTYSTRING)&\\
(1,\EMPTYSTRING)&b&(1)(3,\EMPTYSTRING)&\\
(1,b)&\EMPTYSTRING&(1)(3,\EMPTYSTRING)&\\
(2,\EMPTYSTRING)&a&(2)(9,\EMPTYSTRING)&\\
(2,a)&\EMPTYSTRING&(2)(9,\EMPTYSTRING)&\\
(9,\EMPTYSTRING)&a&(9)(15,\EMPTYSTRING)&\\
(9,a)&\EMPTYSTRING&(9)(15,\EMPTYSTRING)&\\
(9,\EMPTYSTRING)&b&(9)(14,\EMPTYSTRING)&\\
(9,b)&\EMPTYSTRING&(9)(14,\EMPTYSTRING)&\\
(13,\EMPTYSTRING)&d&(13)(17,\EMPTYSTRING)&\\
(13,d)&\EMPTYSTRING&(13)(17,\EMPTYSTRING)&\\
(14,\EMPTYSTRING)&b&(14)(20,\EMPTYSTRING)&\\
(14,b)&\EMPTYSTRING&(14)(20,\EMPTYSTRING)&\\
(15,\EMPTYSTRING)&a&(15)(24,\EMPTYSTRING)&\\
(15,a)&\EMPTYSTRING&(15)(24,\EMPTYSTRING)&\\
(23,\EMPTYSTRING)&b&(23)(26,\EMPTYSTRING)&\\
(23,b)&\EMPTYSTRING&(23)(26,\EMPTYSTRING)&\\
(24,\EMPTYSTRING)&a&(24)(15,\EMPTYSTRING)&\\
(24,a)&\EMPTYSTRING&(24)(15,\EMPTYSTRING)&\\
(24,\EMPTYSTRING)&b&(24)(14,\EMPTYSTRING)&\\
(24,b)&\EMPTYSTRING&(24)(14,\EMPTYSTRING)&\\
(29,\EMPTYSTRING)&d&(29)(31,\EMPTYSTRING)&\\
(29,d)&\EMPTYSTRING&(29)(31,\EMPTYSTRING)&\\
\bottomrule
\end{array}$
\end{minipage}}%


==> figures/fig__subclasses.tex <==
\begin{tabular}{lccccc}
\toprule
&\EPDA&\PDA&\DPDA&\NFA&\DFA\\
\midrule
1-popping&&\Yes&\Yes&\Yes&\Yes\\
deterministic&&&\Yes&&\Yes\\
$\EMPTYSTRING$-step-free&&&&\Yes&\Yes\\
stack-free&&&&\Yes&\Yes\\
\bottomrule
\end{tabular}
